Spectral analysis of the low-mass X-ray pulsar 4U 1822-371: Reflection component in a high-inclination system

The X-ray source 4U 1822-371 is an eclipsing low-mass X-ray binary and X-ray pulsar, hosting a NS that shows periodic pulsations in the X-ray band. The inclination angle of the system is so high that in principle, it should be hard to observe both the direct thermal emission of the central object and the reflection component of the spectrum because they are hidden by the outer edge of the accretion disc. Assuming that the source accretes at the Eddington limit, we analysed non-simultaneous XMM-Newton and NuSTAR observations and studied the average broadband spectrum, with the aim to investigate the presence of a reflection component. No such component has been observed before in a high-inclination source such as 4U 1822-371. We modelled the spectral emission of the source using two different reflection models, Diskline plus Pexriv and the self-consistent model RfxConv. In our analysis, we find significant evidence of a reflection component in the spectrum, in addition to two lines associated with neutral or mildly ionised iron. The continuum spectrum is well fitted by a saturated Comptonisation model and a thermal black-body component emitted by the accretion disc at a lower temperature. We updated the ephemeris, adding two new eclipse times to the most recent ephemeris reported in literature. In our proposed scenario, the source is accreting at the Eddington limit with an intrinsic luminosity of $10^{38}$ erg/s, while the observed luminosity is two orders of magnitude lower. Despite the high inclination, we find that a reflection component is required to fit residuals at the Fe line range and the hard excess observed in the spectrum. The best-fit value of the inner disc radius is still uncertain and model dependent. More observations are therefore needed to confirm these results, which can give important information on this enigmatic and peculiar source.

==> appenix.tex <==
\begin{appendices}
\section{ Other models}
\begin{table}[H]
 \caption{\label{relxill}Comparison of best-fit values for the parameters of the model that includes relxillCp.}
\begin{tabular}{llcccc}

\hline
Model & Component &no-bbody & no-exp& Relxill & nth+Relxill\\
\hline 
{\sc edge} & edgeE(keV) & $9.54 \pm 0.08$ & $9.474 \pm 0.07$ &$9.56^{+0.09}_{-0.08}$ & $9.50 \pm 0.07$ \\
 & MaxTau & 0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.01 &0.08  $\pm$ 0.01 & 0.9 $\pm$ 0.01\\
{\sc TBabs} & nH(10$^{22}$) & $0.08^{+0.02}_{-0.01}$  & $0.211 \pm 0.02$ & $0.11 \pm 0.01$ & $0.13 \pm 0.02$\\ \\

{\sc bbody} & kT(keV) &-& $0.1473^{+0.0062}_{-0.01}$ & $0.203^{+0.008}_{-0.006}$ & $0.208^{+0.007}_{-0.01}$ \\
 & norm(10$^{-4}$) &-& $1.59^{+0.68}_{-0.53}$ & $3.2 \pm 0.2$ & $3.0^{+0.3}_{-0.2}$\\ \\
 
{\sc expabs} (XMM) & LowECut(keV) & $0.185^{+0.08}_{-0.082}$ &-&$2.08^{+0.08}_{-0.15}$&- \\ 
{\sc relxillCp} & Index1 & $0.85^{+0.26}_{-0.29}$ & $1.3^{+0.2}_{-0.3}$ &  $1.38 \pm 0.5$ & $1.09^{+0.3}_{-0.4}$\\
{\sc XMM} & Incl(deg) & 82.5 (frozen)& 82.5 (frozen)& 82.5 (frozen)& 82.5 (frozen) \\
 & Rin & 75 (frozen)  & 75 (frozen)& 75 (frozen)  & 75 (frozen) \\
% & Rout(10$^{3}$) & 1.0 (frozen) \\
 %& z & 0 (frozen) \\
 & gamma & $1.222 \pm 0.005$  & $1.209 \pm 0.002$ & $1.418 \pm 0.004$ & -\\
 & logxi & $0.86^{+0.07}_{-0.05}$ & $1.06^{+0.02}_{-0.03}$ & $1.08 \pm 0.08 $&$1.06^{+0.06}_{-0.04}$\\
% & Afe & 1 (frozen) \\
 & kTe(keV) & $2.92^{+0.03}_{-0.02}$ & $2.87^{+0.02}_{-0.03}$ & $3.4 \pm 0.1 $ & -\\
 & refl$_{frac}$ & $2.9^{+0.3}_{-0.1}$ & $2.5 \pm 0.2$ & $2.8 \pm 0.3$ &-\\
 & norm(10$^{-3}$) & $1.16^{+0.03}_{-0.02}$ & $1.117^{+0.009}_{-0.008}$ & $1.87 \pm 0.08$& $1.0^{+0.3}_{-0.4}$\\
\\

{\sc expabs}(Nu) & LowECut(keV) & 2.63934$_{-0.04}^{+0.23}$&-& 3.0 $\pm 0.1$&-\\
{\sc relxillCp} & Index1 & 0.85 (linked) & 1.3 (linked) & 1.38 (linked)& 1.09 (linked)\\
{\sc NuSTAR} & gamma & $1.51^{+0.03}_{-0.02}$ & 1.39$^{+0.02}_{-0.03}$ & 1.5$^{+0.01}_{-0.03}$ &-\\
 & logxi & $2.70 \pm 0.03$ & 2.0$^{+0.1}_{-0.3}$ & 2.70$^{+0.04}_{-0.03}$ & 2.37 $\pm 0.06$\\
 & kTe(keV) & $4.28^{+0.07}_{-0.06}$ & 4.31$^{+0.10}_{-0.05}$ & 4.17$ \pm 0.07$&- \\
 & refl$_{frac}$ & 2.91 (linked) & 2.5 (linked) &3.5$^{+0.3}_{-0.2}$ &-1 (fixed)\\
 & norm(10$^{-3}$) & $2.42^{+0.08}_{-0.05}$& 1.76$^{+0.07}_{-0.03}$ & 2.43$^{+0.04}_{-0.07}$ & 5.1 $\pm 0.5$\\ \\
 
 {\sc nthComp} & Gamma &-&-&-& $1.248^{+0.009}_{-0.008}$ \\
 {\sc xmm} & kT$_{e}$(keV) &-&-&-&$2.98 \pm 0.04$ \\
 & kT$_{bb}$(keV) &-&-&-& $0.65 \pm 0.04$ \\
 & norm &-&-&-& $0.0109^{+0.0004}_{-0.0003}$ \\
 {\sc nthComp} & Gamma &-&-&-& $1.38^{+0.02}_{-0.04}$ \\
 {\sc nustar} & kT$_{e}$(keV) &-&-&-&$4.25^{+0.07}_{-0.12}$ \\
 & kT$_{bb}$(keV) &-&-&-& $1.1 \pm 0.1$ \\
 & norm ($10^{-3}$ &-&-&-& $7.1 \pm 0.4$ \\
 \\
 \hline 
  {\sc gaussian} & LineE(keV) & $6.514 \pm 0.008$ & $6.512 \pm 0.008$  & $6.512 \pm 0.007$& $6.509 \pm 0.007$\\
{\sc XMM}& Sigma(keV) & 0.075 (frozen) & 0.075 (frozen)& 0.075 (frozen)& 0.075 (frozen) \\
 & norm(10$^{-4}$) & $4.2 \pm 0.2$& $4.4 \pm 0.2$ & $4.6 \pm 0.2$ & $5.1 \pm 0.2$\\
 
 & LineE(keV) & $7.04 \pm 0.02$ & $7.02 \pm 0.02$& $7.04 \pm 0.2$ & $7.02 \pm 0.02$\\
 & Sigma(keV) & 0.075 (linked)& 0.075 (linked)& 0.075 (linked)& 0.075 (linked)\\
 & norm(10$^{-4}$) & $2.6 \pm 0.2$ & $2.5\pm 0.2$& $2.8 \pm 0.2$& $2.73 \pm 0.02$\\ \\
 
 {\sc gaussian} & LineE(keV) & $6.32 \pm 0.03$ & 6.36$\pm 0.02$ & 6.32 $\pm 0.03$ & 6.35 §$\pm 0.02$\\
{\sc NuSTAR}& Sigma(keV) & 0.075 (frozen) & 0.075 (frozen)& 0.075 (frozen)& 0.075 (frozen) \\
 & norm(10$^{-4}$) & $4.4 \pm 0.4$ & 5.6 $\pm 0.4$ & 4.04 $\pm 0.04$ & 4.46 $\pm 0.04$\\
 
 & LineE(keV) & 7.04 (linked)& 7.02 (linked)& 7.04 (linked)& 7.02 (linked) \\
 & Sigma(keV) & 0.075 (linked)& 0.075 (linked)& 0.075 (linked)& 0.075 (linked)\\
 & norm(10$^{-4}$) & $0.9\pm 0.3$ & 1.9$^{+0.4}_{-0.3}$ &0.6 $\pm 0.3$ &1.4$^{+0.3}_{-0.4}$  \\ \\
\hline
 & $\chi^2/dof$ & 3830.3/2935  & 3890.7/2935  & 3472.6/2932 & 3512.5/2932\\
\end{tabular}

\end{table}
\\ \\
\begin{table}[H]
    \centering
 \caption{\label{relxill}Comparison of best-fit values for the parameters of the model that includes relxillCp.}
\begin{tabular}{llcccc}

\hline
Model & Component &no-bbody & no-exp& Relxill & nth+Relxill\\
\hline 
{\sc edge} & edgeE(keV) & $9.54 \pm 0.08$ & $9.474 \pm 0.07$ &$9.56^{+0.09}_{-0.08}$ & $9.50 \pm 0.07$ \\
 & MaxTau & 0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.01 &0.08  $\pm$ 0.01 & 0.9 $\pm$ 0.01\\
{\sc TBabs} & nH(10$^{22}$) & $0.08^{+0.02}_{-0.01}$  & $0.211 \pm 0.02$ & $0.11 \pm 0.01$ & $0.13 \pm 0.02$\\ \\

{\sc bbody} & kT(keV) &-& $0.1473^{+0.0062}_{-0.01}$ & $0.203^{+0.008}_{-0.006}$ & $0.208^{+0.007}_{-0.01}$ \\
 & norm(10$^{-4}$) &-& $1.59^{+0.68}_{-0.53}$ & $3.2 \pm 0.2$ & $3.0^{+0.3}_{-0.2}$\\ \\
 
{\sc expabs} (XMM) & LowECut(keV) & $0.185^{+0.08}_{-0.082}$ &-&$2.08^{+0.08}_{-0.15}$&- \\ 
{\sc relxillCp} & Index1 & $0.85^{+0.26}_{-0.29}$ & $1.3^{+0.2}_{-0.3}$ &  $1.38 \pm 0.5$ & $1.09^{+0.3}_{-0.4}$\\
{\sc XMM} & Incl(deg) & 82.5 (frozen)& 82.5 (frozen)& 82.5 (frozen)& 82.5 (frozen) \\
 & Rin & 75 (frozen)  & 75 (frozen)& 75 (frozen)  & 75 (frozen) \\
% & Rout(10$^{3}$) & 1.0 (frozen) \\
 %& z & 0 (frozen) \\
 & gamma & $1.222 \pm 0.005$  & $1.209 \pm 0.002$ & $1.418 \pm 0.004$ & -\\
 & logxi & $0.86^{+0.07}_{-0.05}$ & $1.06^{+0.02}_{-0.03}$ & $1.08 \pm 0.08 $&$1.06^{+0.06}_{-0.04}$\\
% & Afe & 1 (frozen) \\
 & kTe(keV) & $2.92^{+0.03}_{-0.02}$ & $2.87^{+0.02}_{-0.03}$ & $3.4 \pm 0.1 $ & -\\
 & refl$_{frac}$ & $2.9^{+0.3}_{-0.1}$ & $2.5 \pm 0.2$ & $2.8 \pm 0.3$ &-\\
 & norm(10$^{-3}$) & $1.16^{+0.03}_{-0.02}$ & $1.117^{+0.009}_{-0.008}$ & $1.87 \pm 0.08$& $1.0^{+0.3}_{-0.4}$\\
\\

{\sc expabs}(Nu) & LowECut(keV) & 2.63934$_{-0.04}^{+0.23}$&-& 3.0 $\pm 0.1$&-\\
{\sc relxillCp} & Index1 & 0.85 (linked) & 1.3 (linked) & 1.38 (linked)& 1.09 (linked)\\
{\sc NuSTAR} & gamma & $1.51^{+0.03}_{-0.02}$ & 1.39$^{+0.02}_{-0.03}$ & 1.5$^{+0.01}_{-0.03}$ &-\\
 & logxi & $2.70 \pm 0.03$ & 2.0$^{+0.1}_{-0.3}$ & 2.70$^{+0.04}_{-0.03}$ & 2.37 $\pm 0.06$\\
 & kTe(keV) & $4.28^{+0.07}_{-0.06}$ & 4.31$^{+0.10}_{-0.05}$ & 4.17$ \pm 0.07$&- \\
 & refl$_{frac}$ & 2.91 (linked) & 2.5 (linked) &3.5$^{+0.3}_{-0.2}$ &-1 (fixed)\\
 & norm(10$^{-3}$) & $2.42^{+0.08}_{-0.05}$& 1.76$^{+0.07}_{-0.03}$ & 2.43$^{+0.04}_{-0.07}$ & 5.1 $\pm 0.5$\\ \\
 
 {\sc nthComp} & Gamma &-&-&-& $1.248^{+0.009}_{-0.008}$ \\
 {\sc xmm} & kT$_{e}$(keV) &-&-&-&$2.98 \pm 0.04$ \\
 & kT$_{bb}$(keV) &-&-&-& $0.65 \pm 0.04$ \\
 & norm &-&-&-& $0.0109^{+0.0004}_{-0.0003}$ \\
 {\sc nthComp} & Gamma &-&-&-& $1.38^{+0.02}_{-0.04}$ \\
 {\sc nustar} & kT$_{e}$(keV) &-&-&-&$4.25^{+0.07}_{-0.12}$ \\
 & kT$_{bb}$(keV) &-&-&-& $1.1 \pm 0.1$ \\
 & norm ($10^{-3}$ &-&-&-& $7.1 \pm 0.4$ \\
 \\
 \hline 
  {\sc gaussian} & LineE(keV) & $6.514 \pm 0.008$ & $6.512 \pm 0.008$  & $6.512 \pm 0.007$& $6.509 \pm 0.007$\\
{\sc XMM}& Sigma(keV) & 0.075 (frozen) & 0.075 (frozen)& 0.075 (frozen)& 0.075 (frozen) \\
 & norm(10$^{-4}$) & $4.2 \pm 0.2$& $4.4 \pm 0.2$ & $4.6 \pm 0.2$ & $5.1 \pm 0.2$\\
 
 & LineE(keV) & $7.04 \pm 0.02$ & $7.02 \pm 0.02$& $7.04 \pm 0.2$ & $7.02 \pm 0.02$\\
 & Sigma(keV) & 0.075 (linked)& 0.075 (linked)& 0.075 (linked)& 0.075 (linked)\\
 & norm(10$^{-4}$) & $2.6 \pm 0.2$ & $2.5\pm 0.2$& $2.8 \pm 0.2$& $2.73 \pm 0.02$\\ \\
 
 {\sc gaussian} & LineE(keV) & $6.32 \pm 0.03$ & 6.36$\pm 0.02$ & 6.32 $\pm 0.03$ & 6.35 §$\pm 0.02$\\
{\sc NuSTAR}& Sigma(keV) & 0.075 (frozen) & 0.075 (frozen)& 0.075 (frozen)& 0.075 (frozen) \\
 & norm(10$^{-4}$) & $4.4 \pm 0.4$ & 5.6 $\pm 0.4$ & 4.04 $\pm 0.04$ & 4.46 $\pm 0.04$\\
 
 & LineE(keV) & 7.04 (linked)& 7.02 (linked)& 7.04 (linked)& 7.02 (linked) \\
 & Sigma(keV) & 0.075 (linked)& 0.075 (linked)& 0.075 (linked)& 0.075 (linked)\\
 & norm(10$^{-4}$) & $0.9\pm 0.3$ & 1.9$^{+0.4}_{-0.3}$ &0.6 $\pm 0.3$ &1.4$^{+0.3}_{-0.4}$  \\ \\
\hline
 & $\chi^2/dof$ & 3830.3/2935  & 3890.7/2935  & 3472.6/2932 & 3512.5/2932\\
\end{tabular}

\end{table}

\end{appendices}


==> table/Vecchio_RFX.tex <==
\begin{table}[]\centering
\begin{threeparttable}
\captionsetup{font=small}
 \caption{Best-fit values for the parameters of the three used models. Model 1: $constant\cdot edge\cdot TBabs\cdot(6gaussian+ bbody + relconv\cdot rfxconv\cdot nthComp + nthComp)$, Model 2 has the same components of the Model 1, but in this case the Inner radius R$_{in}$ is let free.} %Model 3: $constant\cdot edge\cdot TBabs\cdot(6gaussian+ bbody + relxillCp + nthComp)$ .}
\begin{tabular}{llcccc}
\toprule
Component & Parameter & Model 1 & Model 2 & Model 3 \\
\toprule 
%{\sc constant} & factor (RGS+FPMA) & 1 (frozen)& \\
%& factor (PN) & 1.04$_{-0.01}^{+0.02}$ \\
%& factor (FPMB) &  1.008$ \pm 0.003$ \\ 
\\
{\sc edge} & E(keV) & $9.44 \pm 0.08$ & 9.50 $\pm 0.08$    \\
 & $\tau$ & 0.075$_{-0.009}^{+0.007}$ & 0.065  $\pm 0.006$ \\
 
{\sc tbabs  } & nH (10$^{22}$) & 0.14 $\pm$ 0.01 &  0.165 $\pm$ 0.003  \\


{\sc bbody} & kT(keV) & $0.197 ^{+0.006}_{-0.009}$& $0.195 \pm 0.002$&  \\
 & norm(10$^{-4}$) & $3.16^{+0.03}_{-0.02}$& $3.42 \pm 0.05$\\ \\
 
{\sc xmm nthComp} & $\Gamma$ & 1.35 $\pm 0.02$& $1.402^{+0.001}_{-0.002}$& 1.35 $\pm 0.02$  \\
 & kT$_{e}$(keV) & $3.4_{-0.2}^{+0.1}$& $3.88 \pm 0.05 $& $3.4_{-0.2}^{+0.1}$ \\
 & kT$_{bb}$(keV) & $0.88^{+0.03}_{-0.05}$ & $0.928 \pm 0.002 & $0.878462^{+0.03}_{-0.05}$ \\
 & norm(10$^{-3}$) & $9.4^{+0.5}_{-0.3}$ & $9.51^{+0.02}_{-0.12}$ & $9.4^{+0.5}_{-0.3}$ \\ \\
 
{\sc nustar nthComp}& $\Gamma$ & 1.537 $_{-0.006}^{+0.008}$ & 1.55 $\pm 0.001$ & 1.537 $_{-0.006}^{+0.008}$ \\
& kT$_{e}$(keV) & $5.02_{-0.05}^{+0.04}$ & $ 5.00 \pm 0.02 $ & $5.02_{-0.05}^{+0.04}$    \\
 & kT$_{bb}$(keV) & $ 0.86 \pm 0.03$ & $ 0.85_{-0.001}^{+0.02}$ & $ 0.86 \pm 0.03$    \\
 & norm(10$^{-2}$) & $1.64_{-0.07}^{+0.01}$ & $ 1.66355_{-0.00027}^{+0.00004}$ & $1.64_{-0.07}^{+0.01}$   \\ \\ 
 
{\sc relconv} & Index & $2.5^{+0.3}_{-0.1}$& $2.1 \pm 0.1 $& $2.5^{+0.3}_{-0.1}$ \\
 & Rbr & 250 (frozen) & 250 (frozen) & 250 (frozen) \\
% & a & 0 (frozen) \\
 & Incl (deg) & 82 (frozen) & 82 (frozen) & 82 (frozen) \\
 & R$_{in}$ & 75\tnote{$\dagger$}&  $15 \pm 3$      & 75\tnote{$\dagger$} \\
& R$_{out}$(10$^{3}$) & 1.0 (frozen) & 1.0 (frozen) & 1.0 (frozen) \\

 {\sc rfxconv} & rel$_{refl}$ & $-0.59^{+0.05}_{-0.07}$& >-0.9& $-0.59^{+0.05}_{-0.07}$ \\
% & Fe$_{abund}$ & 1 (frozen) \\
% & cosIncl & 0.139\\
 & log$_{xi}$ & $2.01^{+0.03}_{-0.30}$& $1.7^{+0.6}_{-0.4}$& $2.01^{+0.03}_{-0.30}$ \\ \\

%{\sc relxillCp} & Index & & & 2.35\tnote{$\dagger$} \\
% & Rbr & & & 250 (frozen) \\
% & a & 0 (frozen) \\
% & Incl(deg) & & & 82\\
% & Rin & &&  ?? \\
% & Rout(10$^{3}$) &&& 1.0 (frozen) \\
% & logxi &&& ?? \\
% & Afe & 1 (frozen) \\
% & refl$_{frac}$ & && ?? \\
% & norm(10$^{-5}$) & && $1.6^{+0.8}_{-0.9}$ \\
 
\hline
\\
{\sc xmm gaussian} & E (keV) & $6.51  \pm 0.01$& $6.51 \pm 0.01$& $6.51 \pm 0.01$   \\
 & $\sigma$ (eV) &<77* & 44* &  \\
 & norm (10$^{-4}$) & $3.5 \pm 0.4$& $3.4\pm 0.2$& $3.5^{+0.3}_{-0.2}$  \\
 \\
 & E (keV) & $7.08 ^{+0.02}_{-0.01}$ & $7.06 ^{+0.02}_{-0.01}$ & $7.08 ^{+0.02}_{-0.01}$ \\
 &  $\sigma$ (eV) & <77& 45$^{2}_{-4}$& <0.07 \\
 & norm (10$^{-4}$) & $2.4 \pm 0.3$ & $2.01 \pm 0.2$ & $2.4 \pm 0.3$  \\
 \\
 {\sc nustar gaussian} & E (keV) & $6.38 \pm 0.02$ & $6.38 \pm 0.02$ & $6.38 \pm 0.02$ \\
 &  $\sigma$ (eV)  & 75\tnote{*}& 75\tnote{*}& 0.075\tnote{*} \\
 & norm (10$^{-4}$) & $4.2 \pm 0.5$&  4.1$^{+0.4}_{-0.3}$& $4.2 \pm 0.5$ \\ \\
 & E (keV)  & 7.08\tnote{*}& 7.06\tnote{*} \\
 &  $\sigma$ (eV) &  $75$\tnote{*} & 75\tnote{*}\\
 & norm (10$^{-4}$) & $0.9\pm 0.4$& $0.5^{+0.3}_{-0.4}$ \\ \\
\hline
 & $\chi^2/dof$ & 3440.36/2933  &  3389.85/2932   \\
 & $\chi^2_{red}$ & 1.17298 & 1.15615  \\ \\ 
 \hline
\hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item [$\dagger$]Kept frozen during the fit.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> table/relxill_vecchio.tex <==
\begin{table}[ht]
 \caption{\label{relxill}Comparison of best-fit values for the parameters of the models that includes different reflection component. \textsc{Model 4A} is defined as $constant\cdot edge\cdot tbabs\cdot(6gaussian+ bbody + expabs \cdot relxillCp)$, while \textsc{Model 4B} has the same components of the \textsc{Model 4A} with the omission of the component \textit{expabs} and the addition of \textit{nthComp}. \textsc{Model 5} is defined as $constant\cdot edge\cdot TBabs\cdot(6gaussian+ bbody + diskline + rdblur\cdot pexrav + nthComp)$.}
 
 \begin{threeparttable}
 
  \resizebox{0.5\textwidth}{!}
  {\begin{minipage}{\textwidth}

\begin{tabular}{llccc}

\hline
Model & Component & Model 4A & Model 4B & Model 5\\
\hline 
{\sc edge} & E(keV) &$9.56^{+0.09}_{-0.08}$ & $9.50 \pm 0.07$ & 9.57$_{-0.08}^{+0.09}$ \\
& $\tau$ &0.08  $\pm$ 0.01 & 0.9 $\pm$ 0.01& 0.08 $\pm 0.01$ \\
{\sc tbabs} & nH(10$^{22}$) & $0.11 \pm 0.01$ & $0.13 \pm 0.02$& 0.12\tnote{*}\\ \\

{\sc bbody} & kT(keV)  & $0.203^{+0.008}_{-0.006}$ & $0.208^{+0.007}_{-0.01}$ & $0.19 \pm 0.003$\\
 & N(10$^{-4}$)  & $3.2 \pm 0.2$ & $3.0^{+0.3}_{-0.2}$& $3.20 \pm 0.06$ \\ \\
 
{\sc expabs} & E$_{Cut}$(keV) &$2.08^{+0.08}_{-0.15}$&-&- \\ 
{\sc relxillCp} & Index  &  $1.38 \pm 0.5$ & $1.09^{+0.3}_{-0.4}$&- \\
{\sc xmm} & Incl(deg) & 82.5\tnote{*}& 82.5\tnote{*}&- \\
 & R$_{in}$ & 75\tnote{*}  & 75\tnote{*}&- \\
% & Rout(10$^{3}$) & 1.0 \tnote{*} \\
 %& z & 0 \tnote{*} \\
 & $\Gamma$  & $1.418 \pm 0.004$ & -& -\\
 & log$_{xi}$  & $1.08 \pm 0.08 $&$1.06^{+0.06}_{-0.04}$& -\\
% & Afe & 1 \tnote{*} \\
 & kTe(keV)  & $3.4 \pm 0.1 $ & -& -\\
 & refl$_{frac}$  & $2.8 \pm 0.3$ &-& -\\
 & N(10$^{-3}$) & $1.87 \pm 0.08$& $1.0^{+0.3}_{-0.4}$ &-\\
\\ 
{\sc expabs} & E$_{Cut}$(keV) & 3.0 $\pm 0.1$&-&-\\
{\sc relxillCp}& $\Gamma$  & 1.5$^{+0.01}_{-0.03}$ &-&-\\
{\sc NuSTAR} & log$_{xi}$  & 2.70$^{+0.04}_{-0.03}$ & 2.37 $\pm 0.06$&-\\
 & kTe(keV)  & 4.17$ \pm 0.07$&-&- \\
 & refl$_{frac}$ &3.5$^{+0.3}_{-0.2}$ &-1\tnote{*}&-\\
 & N(10$^{-3}$)  & 2.43$^{+0.04}_{-0.07}$ & 5.1 $\pm 0.5$&-\\ \\
 
{\sc diskline} & E(keV) &-&-& $6.61 \pm 0.04$   \\
{\sc xmm} & Index  &-&-& $-2.3^{+0.3}_{-0.4}$ \\
 & R$_{in}$  &-&-& 75\tnote{*}   \\
 & Incl(deg)  &-&-& $<62$   \\
 & N (10$^{-4}$)  &-&-& $5.0 \pm 0.5$  \\
 {\sc diskline} & E(keV)  &-&-& $6.52 \pm 0.05$   \\
 {\sc nustar} & Index  &-&-& $ -3.0 \pm 0.8$  \\
 & N (10$^{-4}$)  &-&-& $5.2 \pm 0.7$  \\ \\
 
{\sc pexrav} & rel$_{refl}$ & -&-& -1\tnote{*} \\
% & Fe$_{abund}$ & 1 \tnote{*} \\
 & N$_{xmm}$  &-& -& $0.0547^{+0.0078}_{-0.0088}$ \\
 & N$_{nustar}$  &-& -& $0.24 \pm 0.02$  \\ \\
 

 
 {\sc nthComp} & $\Gamma$ &-& $1.248^{+0.009}_{-0.008}$ & $1.297^{+0.003}_{-0.002}$ \\
 {\sc xmm} & kT$_{e}$(keV) &-&$2.98 \pm 0.04$ & $3.17 \pm 0.03$ \\
 & kT$_{bb}$(keV) &-& $0.65 \pm 0.04$& $0.751^{+0.005}_{-0.01}$ \\
 & N ($10^{-2}$) &-& $1.09^{+0.04}_{-0.03}$ & $1.03 \pm 0.01$ \\
 {\sc nthComp} & $\Gamma$ &-& $1.38^{+0.02}_{-0.04}$ & $1.560 \pm 0.005$\\
 {\sc nustar} & kT$_{e}$(keV) &-&$4.25^{+0.07}_{-0.12}$ & $ 4.97 \pm 0.02$ \\
 & kT$_{bb}$(keV) &-& $1.1 \pm 0.1$& $0.825^{+0.005}_{-0.042}$  \\
 & N ($10^{-3}$) &-& $7.1 \pm 0.4$ & $ 1.5984^{+0.0011}_{-0.0004}$ \\
 \hline 
 \\
  {\sc gaussian} & LineE(keV) & $6.512 \pm 0.007$& $6.509 \pm 0.007$& $6.500 \pm 0.005$\\
{\sc XMM}& Sigma(keV) & 0.075\tnote{*}& 0.075\tnote{*}& 1.8$\times 10^{-17}$\tnote{*} \\
 & N(10$^{-4}$)  & $4.6 \pm 0.2$ & $5.1 \pm 0.2$& $3.0^{+0.2}_{-0.3}$ \\
 & LineE(keV) & $7.04 \pm 0.2$ & $7.02 \pm 0.02$& $7.12^{+0.01}_{-0.02}$\\
 & Sigma(keV) & 0.075\tnote{*}& 0.075\tnote{*}& 1.8\tnote{*}\\
 & N(10$^{-4}$) & $2.8 \pm 0.2$& $2.73 \pm 0.02$& $1.6 \pm 0.3 $\\ \\
 
 {\sc gaussian} & LineE(keV) & 6.32 $\pm 0.03$ & 6.35 $\pm 0.02$& $6.37^{+0.02}_{-0.04}$ \\
{\sc NuSTAR}& Sigma(keV) & 0.075\tnote{*}& 0.075\tnote{*} & 1.8\tnote{*} \\
 & N(10$^{-4}$)  & 4.04 $\pm 0.04$ & 4.46 $\pm 0.04$& $2.5^{+0.5}_{-0.6}$\\
 & LineE(keV) & 7.04\tnote{*}& 7.02\tnote{*}& $7.12$\tnote{*} \\
 & Sigma(keV)& 0.075\tnote{*}& 0.075\tnote{*}& 1.8\tnote{*}\\
 & N(10$^{-4}$) &0.6 $\pm 0.3$ &1.4$^{+0.3}_{-0.4}$  & $<0.3$ \\ \\
\hline
 & $\chi^2/dof$  & 3472.6/2932 & 3512.5/2932  & 3291.1/2929 \\
\end{tabular}
\end{minipage}}

\begin{tablenotes}
\footnotesize
\item[*] Kept frozen during the fit.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> table/time.tex <==
\begin{table}[]\centering
\begin{threeparttable}
  \resizebox{0.5\textwidth}{!}{\begin{minipage}{\textwidth}
\captionsetup{font=small}
 \caption{\label{time} Best-fit values for the parameters of the two models described in the text. \textsc{Model 1} is given by $constant\cdot edge\cdot TBabs\cdot(6gaussian+ bbody + relconv\cdot rfxconv\cdot nthComp + nthComp)$, while \textsc{Model 2} is given by $constant\cdot edge\cdot TBabs\cdot(6gaussian+ bbody + diskline + rdblur\cdot pexriv + nthComp)$. Model 3 has the same components of the Model 1, but in this case the inner radius R$_{in}$ is free to vary. }
\begin{tabular}{lccc}
\toprule
 Parameter & Quadratic & Cubic & LQS  \\
\toprule 
a (s) &         12   \pm 12 & & \\
\hline
\end{tabular}
\end{minipage}}
\begin{tablenotes}
\footnotesize
\item [*]Kept frozen during the fit.
\end{tablenotes}
\end{threeparttable}
\end{table}
